On the profinite rigidity of free and surface groups

Let $S$ be either a free group or the fundamental group of a closed hyperbolic surface. We show that if $G$ is a finitely generated residually-$p$ group with the same pro-$p$ completion as $S$, then two-generated subgroups of $G$ are free. This generalises (and gives a new proof of) the analogous result of Baumslag for parafree groups. Our argument relies on the following new ingredient: if $G$ is a residually-(torsion-free nilpotent) group and $H\leq G$ is a virtually polycyclic subgroup, then $H$ is nilpotent and the pro-$p$ topology of $G$ induces on $H$ its full pro-$p$ topology. Then we study applications to profinite rigidity. Remeslennikov conjectured that a finitely generated residually finite $G$ with profinite completion $\widehat G\cong \widehat S$ is necessarily $G\cong S$. We confirm this when $G$ belongs to a class of groups $\mathcal{H}_{ab}$ that has a finite abelian hierarchy starting with finitely generated residually free groups. This strengthens a previous result of Wilton that relies on the hyperbolicity assumption. Lastly, we prove that the group $S\times {\mathbb Z}^n$ is profinitely rigid within finitely generated residually free groups.

==> bin.tex <==



\section{bin from surface.tex}



Let $S$ be a free or surface group. Recall that if $G$ belongs to the finite, soluble or nilpotent genus of $G$, then  $G$ belongs to the $p$-genus of $S$ by \cref{And}. So the first results of this section about the $p$-genus include all these genera. Before giving the proof of \cref{Remthm} in \cref{Remfree} and \cref{Remsur}, we review a few direct applications of \cref{Tits}.




\begin{cor} \label{ame} Let $G$ be a finitely generated amenable group and let $p$ be a prime. Let $S$ be a free (resp. surface group). Then $G$ belongs to the $p$-genus of $S$ if and only if $G\cong S\cong \Z$ (resp. $G\cong S\cong \Z^2$).
\end{cor}

\begin{proof}  If $S$ is abelian, the conclusion is trivial. So it suffices to prove that if $S$ is non-abelian, then $G$ does not belong to the $p$-genus of $S$. If this was true, we would deduce by \cref{Luck3} that $\b(G)=\b(S)>0$, which would contradict the fact that $G$ is infinite amenable and hence $\b(G)=0$. 
\end{proof}

Alternatively, we note that \cref{ame} is a direct consequence of the Tits alternative of \cref{Tits}. We expect this exact argument to be applied to distinguish the profinite completion of many more groups from the profinite completion of $S$. This applies to some groups acting on 1-manifolds (some of which are non-amenable, by \cite[Theorem 1.4]{Fou21}), as the following result claims.  

\begin{cor}  Let $G$ be a group of piecewise linear homeomorphisms of the interval or a group of piecewise projective homeomorphisms of the real line. Suppose that $S$ is a non-abelian free or surface group. Then $G$ does not belong to the $p$-genus of $S$.
\end{cor}
\begin{proof} By \cref{Tits}, $G$ would contain a non-abelian free subgroup $H$. However,  by \cite[Theorem 1.3]{Fou21}, the second bounded cohomology of $H$ should be 0, which is a contradiction. 
\end{proof}






\section{OTher results}

 It turns out that, as stated, this is not true, as there are finitely generated subgroups $\Ga\inc F_n\times F_n$, when $n\geq 3$, such that the injection induces an isomorphism of profinite completions and $\Ga$ is not isomorphic to $F_n\times F_n$. In particular, it is not hard to see that $\Ga$ cannot be a direct product. This also exhibits that we do not expect $F_n\times F_n$ to be profinitely rigid within finitely generated residually free groups. However, we can restrict our attention to stronger finiteness properties, as in the following result. 

\begin{thmA} \label{prods1} Let $\Ga$ be a residually free group of type $\FP_n$. Suppose that $S_1, \dots, S_n$ are free or surface groups and that $\hat \Ga\cong \hat{S_1}\times \cdots \times \hat S_n$. Then $\Ga\cong S_1\times \cdots \times S_n$. 
\end{thmA}


\section{limit groups}


\section{cohomology}


\begin{thm}[J. Hillman] Let $G$ be a finitely generated $\PD_3$ group. Let $N$ be a finitely generated normal subgroup of infinite index in $G$, then $N$ is a $\PD_2$ group.
\end{thm}


\subsection{Abstract groups}

\begin{thm}[Bieri] Let $G$ be a $\PD_2$ group and let $H$ be an infinite-index subgroup. Then $H$ has cohomological dimension at most one. 
\end{thm}

\begin{thm}[Strebel] Let $G$ be a $\PD_n$ group and let $H$ be an infinite-index subgroup of $G$. Then $H$ has cohomological dimension at most $n-1$.
\end{thm}



\begin{thm} \label{PDv} Let $G$ be a torsion-free group and let $H\leq G$ be a finite-index subgroup. Then  $G$ is $\PD_n$ if and only if $H$ is $\PD_n$. 
\end{thm}

\begin{thm}[Stallings--Swan] Groups of cohomological dimension at most one are free. 
\end{thm}

\begin{thm} Poincar\'e duality groups of dimension two are surface groups. 
\end{thm}


\begin{prop}[\cite{Koc18}, Proposition 2.2] \label{fpseq} Let $1\lrar A\lrar B\lrar C\lrar 1$ be a short exact sequence of groups. Then the following statements are true. 
\begin{enumerate}
    \item If $A$ and $C$ are of type $\FP_n$, then $B$ is of type $\FP_n$.
    \item If $A$ is of type $\FP_n$ and $B$ is of type $\FP_{n+1}$, then $C$ is of type $\FP_{n+1}$. 
\end{enumerate}
\end{prop}

\section{Profinte}

Here we can also recall a few differences between the profinite and pro-$p$ regime. 

\begin{itemize}
    \item Pro-$p$ groups, as opposed to profinite groups, have a Grushko rank equality. 
    \item There is a simple generation criterion for pro-$p$ groups (since the Frattini subgroup is open) but not for profinite groups. In particular, given a group $G$, it is easy to take a minimal set of generators of the pro-$p$ completion belonging to $G$ but not a minimal set of generators of the profinite completion. 
    \item Finitely generated pro-$p$ groups have the form $F\times \Z_p^k$, a simple description. 
    \item Free groups are characterised by a a purely cohomological criterion in the category of pro-$p$ groups (having dimension at most one) but not in the category of profinite groups (as there are projective and non-free profinite groups).
    \item The equivalence between Noetherian condition and ACC is true in pro-$p$ groups but not in full generality.
    \item However, there are a few advantages in considering profinite and not pro-$p$ completions of groups, and one is that fibring is proven to be detected in the former case and splittings are also expected to be detected (while there are many one-ended hyperbolic groups with free pro-$p$ completion). In addition, finite-index subgroups are naturally produced by geometric methods, but having $p$-index is not a well understood condition in terms of geometry. This allows us to understand profinite completions of finite-index subgroups but not their pro-$p$ completions. In fact, one can have parafree group $G$ with a finite-index subgroup with non-free pro-$p$ completion. Moreover, the property of being residually-free is not captured in the $p$-genus either, by the same example as before. 
    \item Following the previous line, there are better separability properties for profinite completions than for pro-$p$ completions. This is also reflected by \cref{indtop2} and \cref{rec0}.
\end{itemize}

\section{Not needed but possibly interesting and wrong}



\begin{prop}\label{trivialmon} Let $G$ be an $\fpi$ group with trivial centre such that $\Ga=G\rtimes \Z$ is coherent. The following are equivalent:
\begin{itemize}
    \item $\Ga$ is residually free.
    \item $G$ is residually free and then the monodromy of $ \Ga$ is trivial.
\end{itemize}
\end{prop}
\begin{proof} One implication is clear. If $G$ is residually free and the monodromy of $\Ga$ is trivial, then $\Ga\cong G\times \Z$ is residually free, too. 

For the reverse implication, we first notice by using \cref{fpseq} that $\Ga$ is of type $\fpi$. By \cref{vprod}, there exist limit groups $G_1$, \dots, $G_n$ and a finite-index $\La\leq \Ga$ such that $\La\cong G_1\times \cdots \times G_n$. Since $\La$ is coherent, it cannot contain a subgroup of the form $F_2\times F_2$. So one of the $G_i$ has to be abelian and infinite. This implies that $\La$ has non-trivial centre. Let $c\in Z( \La)$. For all $x\in \Ga$, there exists $n=|\Ga: \La|$ such that $x^n\in  \La$ and hence $[x^n, c]=1$. By  \cref{Tits0}, this implies that $[x, c]=1$. So $c\in Z(\Ga)$. We write $\Ga=G\rtimes  \lan t \ran$, where $\lan t\ran\cong \Z$. We know that $\Ga$ has non-trivial centre, and we are going to use it to prove that $t\in Z(\Ga)$, which would lead to the desired conclusion. 

Let $(f, t^k)\in Z(\Ga)$, with $f\in G$ and $k\in \Z$. It is clear that $k\neq 0$ because, by assumption, $Z(G)=1$. We consider any $g \in G$. We must have that $(g, 1)$ commutes with $(f, t^k)$, from which we derive that 
\begin{equation}\label{conj}
      g= g^{f t^k} \, \, \mbox{for all $g \in G$.}
\end{equation}

If we apply the previous equation to $g=f$, we deduce that $[f, t^k]=1$, so $[f, t]=1$ by \cref{Tits0}.  We are now ready to prove that $t\in Z(\Ga)$. We proceed by contradiction. Let us take  $g \in G$ such that $[g, t]\neq 1$. Let $F$ be a free group and let $\phi: \Ga\lrar F$ be a group homomorphism such that $\phi([g, t])\neq 1$. As a consequence,  $\phi([g, t^k])\neq 1$, and hence $\phi([g, f])\neq 1$. (WRONG)
\end{proof}


Notice that the following corollary covers one of the cases of \cite{Wil08}. 

\begin{cor}\label{trivialmon1} Let $S$ be a free or surface group. Suppose that $\Ga=S\rtimes \Z$ is residually free. Then the monodromy of $\Ga$ is trivial and hence $\Ga\cong S\times \Z$. 
\end{cor}
\begin{proof}
If $S$ is free, then $\Ga$ is coherent by . If $S$ is a surface group, then $\Ga$ is a 3-manifold group and hence it is coherent by \cite{Sco73}. In any case, the conclusion follows from \cref{trivialmon}.
\end{proof}


It may be interesting to still pose the following two questions. 

 \begin{question} Let $G$ be a limit group. Is $G\rtimes \Z$ coherent? 
 \end{question}
 The previous would imply that the only way $G\rtimes \Z$ is residually-free (with $G$ being limit) is when the monodromy is trivial. 
 \begin{question} Let $G$ be LERF. Is it true that $G\times  \Z$ is LERF?
 \end{question}

\section{profinite groups}

Surprisingly, there are scenarios where we can relate finiteness properties of the profinite or pro-$p$ completion of groups to the groups themselves. For this to be done when we study the $p$-genus of groups $S\times \Z^n$, where $S$ is a free or hyperbolic surface, we shall first understand finiteness properties of their pro-$p$ completions, and we leave the following simple (but useful) lemma at hand.

\begin{lemma} \label{pFP}
Let $S$ be a free or hyperbolic surface and let $\GG$ be the pro-$p$ completion of $S\times \Z^n$. Then any closed finitely generated subgroup of $\GG$ is of type $p-\fpi$. 
\end{lemma}
\begin{proof} The finitely generated profinite group $\GG$ is a closed subgroup of $S_{\hp}\times \Z_p^n$. We consider the natural projection $p: S_{\hp}\times \Z_p^n\lrar S_{\hp} $. Then there is a short exact sequence $1\lrar \Z_p^n\cap \GG \lrar \GG\lrar p(\GG)\lrar 1$. By \cref{fpseq}, it is enough to show that both $\Z_p^n\cap \GG$ and $p(\GG)$ are of type $p-\fpi$. The group  $\Z_p^n\cap \GG$ is isomorphic to $\Z_p^k$ for some $k$, so this case is clear. For the group $p(\GG)$, we observe that it is a finitely generated closed subgroup of the $\PD_2$ pro-$p$ group $S_{\hp}$. If it has finite index, then the assertion follows. If it is infinite index, then by \cref{Serre}, it is free and thus of type $\fpi$. 
\end{proof}

\section{unneeded betti}

One of the aims of this paper consists on finding some structure on a group from its profinite or pro-$p$ completion. \cref{bettieq} claims that in many cases we can detect first $L^2$ Betti numbers (and, for example, the vanishing of these numbers gives information about the group, as in \cref{fibring}). Another motivation would now be giving a simple criterion that ensures the vanishing of the first $L^2$ Betti number of groups. 

\begin{thm}[\cite{Gab02}, Theorem 6.8] \label{0Betti} Suppose that 
\[1 \rar N\rar G \rar G' \rar 1\]
is an exact sequence of groups where $N$ and $G'$ are infinite. If $b_1^{(2)}(N)<\infty$ (for example, $N$ is finitely generated) then $b_1^{(2)}(G)=0$. 
\end{thm}

\section{Not needed technical lemmas about cubulations}


\begin{defi} We say that a group is co-compactly cubulated if it acts properly and co-compactly on a CAT(0) cube complex. 
\end{defi}

The following is a particular case of theorem A of \cite{Hsu15}.

\begin{thm}[Co-compactly cubulating malnormal amalgams]  Let $G=A\underset{C}{*} B$ (or $G=A\underset{C}{*}$) be a hyperbolic group, where $C$ is malnormal and quasi-convex in $G$. If $A$ and $B$ (or $A$) act properly, cocompactly and virtually specially on a CAT(0) cube complex, then so does $G$. 
\end{thm}

As a direct consequence, we can rephrase
\begin{cor}[Co-compactly cubulating cyclic amalgams] \label{hsu} Let $G=A\underset{C}{*} B$ (or $G=A\underset{C}{*}$) be a torsion-free hyperbolic group, where $C$ is an infinite cyclic subgroup. If $A$ and $B$ (or $A$) act properly, cocompactly and virtually specially on a CAT(0) cube complex, then so does $G$. 
\end{cor}

We recall that sometimes, under hyperbolicity assumptions, we ensure virtual speciality for geometric actions by the follo \cite[Theorem 1.1]{Ago13}.
\begin{thm} \label{Agol} Let $G$ be a hyperbolic group acting properly and cocompactly on a CAT(0) cube complex. Then $G$ has a finite-index subgroup acting specially on $X$. 
\end{thm}


\begin{prop}[Inadequate proof, because it's easier than this] If $G$ is in the $p$-genus of $S\times \Z^n$, then abelian subgroups are finitely generated. 
\end{prop}
\begin{proof}We define a filtration of $G_{\hp}$ by closed normal subgroups as follows. We set $\GG_0=1$ and $\GG_{k}=S_{\hp}\times \Z_p^{k-1}$ for $1\leq k\leq n+1$, where $\GG_k$ corresponds to the first $k$ coordinates of $G_{\hp}\cong S_{\hp}\times \Z_p^n$ when seen as a direct product of $S_{\hp}$ and $n$ copies of $\Z_p$. The subsequent quotients $\GG_{i+1}/\GG_i$ are isomorphic to $S_{\hp}$ if $i=0$ and to $\Z_p$ otherwise. We consider now a filtration of $A$ by taking $A_k=A\cap \GG_k$ for all $0\leq k\leq n+1$. 
    
    For all $k\geq 1$, there is a continuous retraction $r_k:  \GG_{k+1}\lrar \GG_k$  consisting on projecting canonically onto the first $k$ coordinates of $\GG_{k+1}$, so its kernel $\KK_k$ is isomorphic to $\Z_p$. If we restrict this retraction to $A_{k+1}$, we get a retraction $r_{k}: A_{k+1}\lrar A_k$ whose kernel $K_k$ is contained in $\KK_k$. We want to show that $K_k$ is cyclic. This will be a consequence of \cref{cyclic} once we prove that $K_k$ is locally cyclic. Let $B_k\leq K_k$ be a finitely generated subgroup. By applying part (1) of the theorem to $B_k$, we derive that the natural map $\left(B_k\right)_{\hp}\lrar G_{\hp}$ is injective. Moreover, the image of the previous map is $\ove B_k\sub \ove K_k\sub \KK_k\cong \Z_p$. So there is an injection $\left(B_k\right)_{\hp}\inc \Z_p$, implying that the pro-$p$ completion of $B_k$ is cyclic. Since $B_k$ is finitely generated and residually-$p$, it follows that $B_k$ is cyclic. In conclusion, $K_k$ is locally cyclic, as we wanted. 
    
    Once we know that $K_k$ is cyclic for $k\geq 1$, it will follow that $A_{k+1}$ is finitely generated if we prove that $A_k$ is finitely generated. So in order to conclude that $A$ is finitely generated it only remains to prove that $A_1$ is finitely generated. In fact, by part (1) of this theorem, for all finitely generated $B_0\leq A_1$, there is an injection $\left(B_0\right)_{\hp}\inc \ove{B_0}\sub \ove{A_1}\sub S_{\hp}$, so we deduce from \cref{subabprof} that the pro-$p$ completion of $B_0$ is cyclic. So $A_1$ is locally cyclic and, again by \cref{cyclic}, it is cyclic. 

\end{proof}


\begin{remark} 
At some point I confused the cohomological goodness, which implies $\cd_p(G)=\cd_p(\hat G)$, with the following property: $\cd_p(G)=\cd_p(G_{\hp})$. However, one can take the double of a free group of rank two $F=F(a, b)$ along $a^2b^3$ and observe that the resulting double $G$ is a non-free hyperbolic limit and parafree group. So $G$ is cohomological good, $G_{\hp}$ is free and it contains a surface as a virtual retract. 

I was also using incorrectly that $\cd_p$ is monotone in abstract subgroups. 

\end{remark}

\subsection{More trash about products of limit groups and free abelian groups}
However, if we look at the profinite completion instead of the pro-$p$ completion for a single prime $p$, we do not need to include the condition on $\fpi$. 

\begin{cor} Let $G$ be a finitely generated residually free group with the same profinite completion as $F\times \Z^n$. Then $G\cong F\times \Z^n$. 
\end{cor}

We can prove an analogous statement for the surface case. 

\begin{thm} Let $G$ be a finitely generated residually free group with the same profinite completion as $\pi_1\Sg\times \Z^n$. Then $G\cong \pi_1\Sg\times \Z^n$.
\end{thm}


We shall remark why determining the groups $S\times \Z^n$, for a free or surface $S$, is harder than determining $F$ or $S$ itself. 

\begin{prop} Suppose that $\mathcal F$ be family of groups that contains free and surface groups and it is closed under the operation of taking direct products. Suppose that $S\times \Z^n$ is profinitely rigid within $\mathcal F$. Then $S$ is profinitely rigid within $\mathcal F$. 
\end{prop}

\begin{proof} Suppose that $G\in \mathcal F$ is residually finite and $\hat G\cong \hat S$. Then $G\times \Z^n\in \mathcal F$ has the same profinite completion as $S\times \Z^n$ and is residually finite. So  $G\times \Z^n\cong S\times \Z^n$. If $S$ is abelian, it is clear that this implies that $G\cong S$. Otherwise, $S$ is centreless and hence $G\cong G\times \Z^n/Z(G\times \Z^n)\cong S\times \Z^n/Z(S\times \Z^n)\cong S. $
\end{proof}

It is tempting to try and extend these results by replacing the free or surface groups by other hyperbolic limit groups $L$. However, before doing that, we should be able to determine $L$ within hyperbolic limit groups by looking at the profinite completion, and this question seems still out of reach. Still, we can prove the following. 

\begin{thm} Let $L$ be a hyperbolic limit group such that $L_{\hp}$ is SRN for some prime $p$. Let $G$ be a finitely generated group. Then the following is equivalent.
\begin{itemize}
    \item  $G$ is residually free and has the same profinite completion as $L\times \Z^n$. 
    \item $G$ is isomorphic to $L'\times \Z^n$, where $L'$ is a hyperbolic limit group with the same profinite completion as $L$.
\end{itemize}
\end{thm}


\begin{question} Do pro-$p$ completions of hyperbolic limit groups have the property that they do not contain $\Z_p^2$? Also, how compatible is their finite cyclic hierarchy with pro-$p$ completions? If the former question has positive answer, then these are SRN. 
\end{question}



\subsection{Nilpotent section extra comments}


\begin{eg}\label{badpoly} There is a version of this result for polycyclic groups \cite[Theorem 1 and comments below]{Lea64}, which says that these groups are residually-$P$ for a finite set of primes $P$. However, the description of this primes is not as explicit as in \cref{resp}, as they may not relate in any way the torsion of elements. This is seen in the following two examples. 
\begin{itemize}
    \item Let $\Z/p$ be the cyclic group of order $p$ generated by $a$. Let $\Z$ be an infinite cyclic group generated by $b$. The automorphism group of $\Z/p$ is isomorphic to $\Z/(p-1)$. We consider an action of $\Z$ on $\Z/p$ for which $b$ acts in $\Z/p$ as a generator of $\Aut (\Z/p)$. We form the semidirect product $G_1=\Z/p\Z\rtimes \Z$. Then $G_1$ is not residually nilpotent. In fact, the commutator  $ [a, b]$ is a non-trivial element of $\lan a\ran$, so $\lan a\ran\sub \ga_k G_1$ for all $k$. 
    \item Let $G_2$ be the fundamental group of the Klein bottle, with presentation $G_2=\lan a, b| abab^{-1}\ran$. Then $G_2$ is $\Z$-by-$\Z$ and it is torsion-free polycyclic of Hirsch length 2. When $p\neq 2$, its pro-$p$ completion is isomorphic to $\Z_p$, which is abelian. So $G_2$ cannot embed into its pro-$p$ completion and so it is not residually-$p$ for any $p\neq 2$. 
\end{itemize}

\end{eg}
There is no hope in trying to generalise \cref{pMalcev} to more general polycyclic groups. In fact, the next simple class of these examples that are not nilpotent are polycyclic groups of Hirsch length equal to 2, and none of the examples of \cref{badpoly} verify \cref{pMalcev}. In the first example, any normal subgroup of finite-index of $G_1$ intersects $\lan b\ran\cong \Z$ in a subgroup of index divisible by $p-1$. In particular, if $p\geq 5$, then the pro-$q$ topology of $G_1$ does not induce in $\lan b\ran$ its full pro-$q$ topology for all primes $q$. Secondly, $G_2$ has a 2-index subgroup $H_2$ isomorphic to $\Z^2$, but the pro-$p$ completion of $G_2$ is isomorphic to $\Z_p$ if $p\geq 3$, so it cannot contain $\Z_p^2$, implying that the pro-$p$ topology of $G_2$ does not induce in $H_2$ its full pro-$p$ topology for $p\geq 3$.



\subsection{Rigidity of surfaces among certain splittings}


\begin{thm} Let $g\geq 0$ be an integer and let $G=A\underset{H}{*} B$ be an amalgamated product of groups with $d(A)+d(B)=2g$. Suppose that $G$ is cohomologically good. Then $G$ belongs to the finite genus of $\pi_1\Sg$ if and only if $G\cong \pi_1 \Sg$. 
\end{thm}

Given a group in the finite genus of a surface group, it is clear that it has to be one-ended. It is now natural to consider the JSJ decomposition and relate it to JSJ decompositions of the surface getting rid of useless relations by making use of the classification of Demushkin groups. This is what we did in a very particular case. 

We can make another comment regarding JSJ decompositions and the finite genus of surfaces. There is a general theory of these splittings when one sometimes considers a more general of small edge subgroups, such as slender groups. By the strong Tits alternative, non-trivial slender subgroups are necessarily isomorphic to $\Z$. 

These ideas suggest that the difficult case may lie in the case of rigid groups (those with no splitting at all). This was already the case from an alternative viewpoint. Certainly, an important idea in these arguments is to ensure the existence of surfaces. Wilton reduces Gromov questions on one-ended torsion-free hyperbolic groups to rigid ones. (wait for torsion-free hyperbolic groups contain quasi-embedded infinite cyclic groups, and these are rigid).

\begin{thm} Let $G$ be the fundamental group of a finite graph of groups with virtually free groups and virtually cyclic edge subgroups. Suppose that $G$ belongs to the finite genus of $\pi_1\Sg$. Then $G\cong \pi_1 \Sg$. 
\end{thm}
\begin{proof} It is clear that $G$ is torsion-free, so its edges are free and its edges are either trivial or infinite cyclic (however, the first case cannot occur because $G$ is one-ended). On the other side, by the Tits property, the centralisers of $G$ are cyclic, and hence $G$ is hyperbolic. By Wilton, it contains an quasi-convex embedded surface $\pi_1\Sg$. Moreover, since $G$ is hyperbolic virtually special, then this surface is a virtual retract. 
\end{proof}

\begin{thm} Let $G$ be the fundamental group of a finite graph of groups $(\G, Y)$ and let $\Sg$ be a closed orientable surface. Suppose that $G$ is good and that
\[\sum_{v\in V(Y)}  d(\G(v))=1+|E(Y)|+ \chi(\Sg).\]
If $\hat G\cong \hat{\pi_1\Sg}$, then $G\cong \pi_1\Sg$. In fact, in that case, $(\G, Y)$ must be a extension of free groups over cyclic subgroups. 
\end{thm}

\begin{eg} The previous result would say that given a good and residually finite amalgamated product $A\underset{H}{*}B$ with $d(A)+d(B)=2g$, where $g$ is the genus of a closed orientable surface $ \Sg$, then $\hat{G}\cong\hat{\pi_1\Sg}$ if and only if $G\cong \pi_1\Sg$. 
\end{eg}

\section{surface section}

\begin{remark}
There exist limit parasurface groups $G$ that are not isomorphic to surfaces. It is enough to take the double of the free group in $F$ even number of generators along the word $[a_1, a_2\delta]\cdots [a_{n-1}, a_{n}]$. 
\end{remark} 


\section{p-genus complicated arguments}


\begin{proof}[Proof of \cref{fpi-p}] On the first place, we remark that the statement is trivial when $S$ is abelian, since $G$ would be isomorphic to $S\times \Z^n$ in that case. So we are going to consider the cases when $S$ is non-abelian free or a hyperbolic surface group. 

We divide the proof in several claims and, first, we introduce a definition that will be helpful for the purpose of the proof and unravelling some hidden structure in the given group $G$. We say that a sequence of pairs $(G_i, H_i)$ of subgroups of $G$ with range $0\leq i\leq m$ is a {\te fibring sequence of length $m+1$} if for all $1\leq i\leq m$, the following is true: 
\begin{enumerate}
    \item $G_0=G$.
    \item $H_i$ has finite index in $G_i$.
    \item For $i<m$, $H_i=G_{i+1}\rtimes \Z$.
\end{enumerate}
\begin{claim} \label{01} There exists a fibring sequence of length $n$ in $G$.
\end{claim}
For proving this, we first notice that there is such a sequence of length $m=0$ just by taking $G_0=H_0=G$. Secondly, we prove that whenever we are given a fibring sequence of length $m<n$, we can possibly modify $H_m$ and add $G_{m+1}$ and $H_{m+1}$ to the sequence so we have a fibring sequence of length $m+1$. For this, it is enough to prove that given such a sequence of length $m<n$, $G_m$ has to be virtually fibred (since then we could just re-define $H_m$ to be any finite-index subgroup $G_m$ that fibres and take $G_{m+1}=H_{m+1}$ to be the kernel of some fibration $G_m\lrar \Z$). To prove that $G_m$ is virtually fibred we apply \cref{fibring}, for which we need to check that $G_m$ is RFRS and that $\b(G_m)=0$. The former follows from the fact that $G_m$ is a subgroup of $G$ and that this is RFRS by \cref{pRFRS}. In addition, we notice that, by induction on $i$, there is an injection $\Z^{n-i}\inc Z(G)\cap G_i$, so $Z(G_m)\neq \{1\}$ as $m<n$ and hence, by \cref{0Betti}, it would follow that $\b(G_m)=0$. So we need to check by induction that $\Z^{n-i}\inc Z(G)\cap G_i$. The case $i=0$ is just a consequence of \cref{Titsn}, since $Z(G)\cong \Z^n$ and $G_0=G$. If we have proven for some $0 \leq i\leq m-1$ that $ Z(G)\cap G_i$ contains a subgroup $A_i\cong \Z^{n-i}$, we notice that $B_i=A_i\cap H_i\cong \Z^{n-i}$ is contained in $H_i$ and we look at the projection of $\phi_i: H_i\lrar \Z$ with kernel $G_{i+1}$. There is a short exact sequence $1\lrar B_i\cap G_{i+1}\lrar H_i\lrar \phi_i(B_i)\lrar 1$, where $\phi_i(B_i)\leq \Z$ has rank at most one, so the rank of  the free abelian group  $B_i\cap G_{i+1} $ must be at least $n-i-1$, and thus $B_i\cap G_{i+1}\leq Z(G)\cap G_{i+1}$ contains $\Z^{n-i-1}$, as we wanted. \cref{01} is proven.



Now that we have proven its existence, we can consider a fibring sequence of length $n$ in $G$. 

We consider the closures $\ove G_i$ and $\ove H_i$ of $G_i$ and $H_i$, respectively, in the pro-$p$ completion $G_{\hp}\cong S_{\hp}\times \Z_p^n.$ By \cref{pFP}, these closed subgroups are of type $p-\fpi$. 


\begin{claim} \label{02} If $S$ is free, then $\cd_p(\ove G_i)= n+1-i$ for all $0\leq i\leq n$. If $S$ is a hyperbolic surface group, then $\ove G_i$ is $\PD_{n+2-i}$ for all $0\leq i\leq n$, and it is not virtually soluble. 
\end{claim}

 We can prove the statement by induction on $i$. Let us first consider the case when $S$ is free. We know that $G_0=G$, so $\ove{G}=G_{\hp}$ has $\cd_p=n+2$. Suppose that  $\cd_p(\ove G_i)= n+1-i$ for some $0\leq i\leq n-1$. By \cref{cdopen}, $\cd(\ove{H_i})=\cd_p(\ove G_i)=n+1-i$. We have that $\ove{H_i}=\ove{G_{i+1}}\rtimes \Z_p$. By \cref{wz04}, $\cd_p(\ove{G_{i+1}})=\cd_p(\ove{H_i})-1=n-i$, and the induction step is complete. The exact same proof can also say, even when $S$ is a surface, that $\cd_p(\ove{G_i})<\infty$ for all $i$. 
 
 Now we consider the case when $S$ is a hyperbolic surface group. The base of the induction $i=0$ is trivial and says that $\ove{G_0}=G_{\hp}$ is $\PD_{n+2}$ and is not virtually soluble (which is clear because one of its quotients, $S_{\hp}$, is not virtually soluble either). Suppose that $\ove{G_i}$ is $\PD_{n+2-i}$ for some $0\leq i\leq n-1$ and that it is not virtually soluble. Then these two properties clearly pass to the open subgroup $\ove{H_i}$ by \cref{virPD}. Now we write $\ove{H_i}=\ove{G_{i+1}}\rtimes \Z_p$. By \cref{PDsec}, $\ove{G_{i+1}}$ is $\PD_{n+1-i}$. In addition, since the extension of virtually soluble groups is, again, virtually soluble, then $\ove{G_{i+1}}$ cannot be virtually soluble either. The induction step is complete and \cref{02} is proven. 
 
 
\begin{claim} \label{03} The group $G_n$ is limit.  
\end{claim}
By \cref{lim}, it is enough to show that the finitely generated residually free group $G_n$ has no $\Z^2$. 
Consider first the case when $S$ is free. By \cref{02}, $\cd_p(\ove{G_n})=1$ is free and it cannot contain $\Z_p^2$. If $G_n$ contained $\Z^2$, then the injection $\Z^2\inc G_n$ would induce an injection $\Z_p^2\inc \ove{G_n}\sub G_{\hp}$ by \cref{Titsn}, which would result in a contradiction. 

When $S$ is a hyperbolic surface, we observe instead that any injection $\Z^2\inc G$ would induce by \cref{Titsn} an injection $\Z_p^2\inc \ove{G_n}$, which is $\PD_2$. Simultaneously, $\ove{G_n}$ is not virtually soluble by \cref{02}, so the previous injection should have an image of infinite index. Hence, by \cref{Serre}, $2=\cd_p(\Z_p^2)<\cd_p(\ove{G_n})=2$, which would be absurd. The proof of \cref{03} is complete. 

We know that $G_n$ is limit and so it is $\fpi$. We are now ready to finish the proof of the theorem. We prove by induction on $j$, with range $0\leq j\leq n$, that $G_{n-j}$ is $\fpi$. The base case $j=0$ is already verified. If we knew that $G_{n-j}$ is $\fpi$ for some $0\leq j\leq n-1$, then $H_{n+1-j}=G_{n-j}\rtimes \Z$ would be $\fpi$ by \cref{fpseq}. In addition, since $G_{n+1-j}$ is torsion-free and contains $H_{n+1-j}$ as a finite-index subgroup, then, by \cref{PDv}, $G_{n+1-j}$ is also $\fpi$. This completes the induction step and also the proof of the theorem. 
\end{proof}
